SCDE: Sentence Cloze Dataset with High Quality Distractors From Examinations

We introduce SCDE, a dataset to evaluate the performance of computational models through sentence prediction. SCDE is a human-created sentence cloze dataset, collected from public school English examinations. Our task requires a model to fill up multiple blanks in a passage from a shared candidate set with distractors designed by English teachers. Experimental results demonstrate that this task requires the use of non-local, discourse-level context beyond the immediate sentence neighborhood. The blanks require joint solving and significantly impair each other's context. Furthermore, through ablations, we show that the distractors are of high quality and make the task more challenging. Our experiments show that there is a significant performance gap between advanced models (72%) and humans (87%), encouraging future models to bridge this gap.

==> sections/background.tex <==
\subsection{Problem Complexity}
Let $n$ be the number of candidates and $b$ the number of blanks. For our case, with a typical $n=7$ and $b=5$, the size of the answer space, $|A|$ is given by
\begin{align*}
    |A| &= C(n,b) \times b! \\
        &= C(7,5) \times 5! \\
        &= \frac{7(7-1)}{2} \times 120 \\
        &= 2520
\end{align*}
Thus, the \% chance of guessing all passage blanks exactly right at random is very low, precisely,  $\frac{1}{2520} \times 100 = 0.03\%$. 

What are the chances of getting answers partially correct? In particular, consider the number of answer permutations which get  atleast one blank correct, denoted by $\zeta(n,b)$. If we have the same number of candidates as blanks, this is equivalent to $b! - D_{b}$, where $D_{b}$ is the number of derangements\footnote{\url{en.wikipedia.org/wiki/Derangement}} of $b$ elements. In the presence of more candidates than blanks i.e distractors, this expression becomes more involved to derive. We defer the derivation to Appendix \S 1.2 for paucity of space. With $n=7$ and $b=5$, $\zeta(n,b)=1306$, or $51.8\%$. In other words, there is a $48.17$\% probability of being entirely wrong with a randomly chosen set of answers to each blank in the passage. \xiang{I will add derivation to the appendix.}
